Learning to Prove Safety over Parameterised Concurrent Systems (Full Version)

We revisit the classic problem of proving safety over parameterised concurrent systems, i.e., an infinite family of finite-state concurrent systems that are represented by some finite (symbolic) means. An example of such an infinite family is a dining philosopher protocol with any number n of processes (n being the parameter that defines the infinite family). Regular model checking is a well-known generic framework for modelling parameterised concurrent systems, where an infinite set of configurations (resp. transitions) is represented by a regular set (resp. regular transducer). Although verifying safety properties in the regular model checking framework is undecidable in general, many sophisticated semi-algorithms have been developed in the past fifteen years that can successfully prove safety in many practical instances. In this paper, we propose a simple solution to synthesise regular inductive invariants that makes use of Angluin's classic L* algorithm (and its variants). We provide a termination guarantee when the set of configurations reachable from a given set of initial configurations is regular. We have tested L* algorithm on standard (as well as new) examples in regular model checking including the dining philosopher protocol, the dining cryptographer protocol, and several mutual exclusion protocols (e.g. Bakery, Burns, Szymanski, and German). Our experiments show that, despite the simplicity of our solution, it can perform at least as well as existing semi-algorithms.

==> inferring.tex <==
%% 2 pages
%% Describe the algorithm
%%

==> optimizations.tex <==
%% 2 pages
%% Optimizations
%%

==> pic1.tex <==
\begin{tikzpicture}
\tikzset{every state/.style={minimum size=15pt}}
\node[initial,state] (A) {};
\node[state,accepting] (B) [right =2em of A] {};

\tikzset{loop/.style={in=50,out=130, looseness=5}}
\draw[->,loop above] (B) to node[above] {$N$} (B);
\draw[->] (A) to node[above]{$T$}(B);
\end{tikzpicture}

==> table3.tex <==
\begin{table}[htb]
\begin{center}
\scalebox{0.8}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline 
 & \textsf{\footnotesize{}\#}\textsf{\tiny{}label} & \textsf{\footnotesize{}S}\textsf{\tiny{}init} & \textsf{\footnotesize{}T}\textsf{\tiny{}init} & \textsf{\footnotesize{}S}\textsf{\tiny{}trans} & \textsf{\footnotesize{}T}\textsf{\tiny{}trans} & \textsf{\footnotesize{}S}\textsf{\tiny{}bad} & \textsf{\footnotesize{}T}\textsf{\tiny{}bad} & \textsf{\footnotesize{}\#}\textsf{\tiny{}member} & \textsf{\footnotesize{}\#}\textsf{\tiny{}equiv} & \textsf{\footnotesize{}Q}\textsf{\tiny{}size} & \textsf{\footnotesize{}C}\textsf{\tiny{}size} & \textsf{\footnotesize{}Time}\tabularnewline
\hline 
\hline 
Bakery & 3 & 3 & 3 & 5 & 19 & 3 & 9 & 147 & 6 & 5 & 4 & 0.0s\tabularnewline
\hline 
Burns & 12 & 3 & 3 & 10 & 125 & 3 & 36 & 1063 & 8 & 5 & 3 & 0.2s\tabularnewline
\hline 
Szymanski & 11 & 9 & 9 & 118 & 412 & 13 & 40 & 160742 & 25 & 14 & 12 & 0.3s\tabularnewline
\hline 
German & 581 & 3 & 3 & 17 & 9487 & 4 & 2112 & 348499 & 13 & 6 & 4 & 4.8s\tabularnewline
\hline 
Dijkstra & 42 & 1 & 1 & 13 & 827 & 3 & 126 & 4756 & 9 & 4 & 2 & 0.1s\tabularnewline
\hline 
Dijkstra ring & 12 & 3 & 3 & 13 & 199 & 3 & 36 & 6112 & 14 & 7 & 4 & 1.4s\tabularnewline
\hline 
Dining crypto. & 14 & 10 & 30 & 17 & 70 & 12 & 70 & 11443 & 19 & 7 & 5 & 0.1s\tabularnewline
\hline 
Coffee can & 6 & 8 & 18 & 13 & 34 & 5 & 8 & 48 & 3 & 3 & 2 & 0.0s\tabularnewline
\hline 
Herman linear & 2 & 2 & 4 & 4 & 10 & 1 & 1 & 5 & 2 & 2 & 1 & 0.0s\tabularnewline
\hline 
Herman ring & 2 & 2 & 4 & 9 & 22 & 1 & 1 & 5 & 2 & 2 & 1 & 0.0s\tabularnewline
\hline 
Israeli-Jalfon & 2 & 3 & 6 & 24 & 62 & 1 & 1 & 38 & 4 & 3 & 2 & 0.0s\tabularnewline
\hline 
Lehmann-Rabin & 6 & 4 & 4 & 14 & 96 & 3 & 13 & 545 & 7 & 7 & 5 & 0.1s\tabularnewline
\hline 
LR philo. & 4 & 4 & 4 & 3 & 10 & 3 & 4 & 74 & 3 & 6 & 3 & 0.0s\tabularnewline
\hline 
mux array & 6 & 3 & 3 & 4 & 31 & 3 & 18 & 204 & 5 & 5 & 3 & 0.0s\tabularnewline
\hline 
Res. allocator & 3 & 3 & 3 & 7 & 25 & 4 & 9 & 110 & 5 & 5 & 3 & 0.0s\tabularnewline
\hline 
Kanban & 3 & 25 & 48 & 98 & 250 & 37 & 68 & {\small{}\textgreater{}}455554 & {\small{}\textgreater{}}28 & {\small{}\textgreater{}}44 & {\small{}\textgreater{}}28 & {\small{}\textgreater{}}60s\tabularnewline
\hline 
Water jugs & 11 & 5 & 6 & 23 & 132 & 5 & 12 & 27468 & 23 & 7 & 5 & 0.1s\tabularnewline
\hline 
\end{tabular}}
\end{center}
\hspace{2em} \caption{Some statistics of models and experiments. \textsf{\footnotesize{}
		\#}\textsf{\tiny{}label} is the size of alphabet,\textsf{\footnotesize{}
		S}\textsf{\tiny{}x} and\textsf{\footnotesize{} T}\textsf{\tiny{}x}
	stand for the numbers of states and transitions, respectively, in
	the automaton/transducer representing the initial configurations,
	transitions, and bad configurations for \textsf{\footnotesize{}X}
	being \textsf{\footnotesize{}init}, \textsf{\footnotesize{}trans},
	and \textsf{\footnotesize{}bad}, respectively. Columns \textsf{\footnotesize{}\#}\textsf{\tiny{}member}
	and \textsf{\footnotesize{}\#}\textsf{\tiny{}equiv} stand for the
	numbers of membership queries and equivalence queries, respectively,
	made by our implementation. Columns\textsf{\footnotesize{}
		Q}\textsf{\tiny{}size} and\textsf{\footnotesize{} C}\textsf{\tiny{}size}
	stand for the maximum sizes of query strings and counterexamples,
	respectively, that have appeared in the learning process. Finally,\textsf{\footnotesize{}
		Time} records the execution time of our prototype for each example.}\label{tab:more_data}
\end{table}

==> table4.tex <==
\begin{wraptable}{r}{7cm}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{|l|c|c|c||c|c|c||c|}
\hline 
 & \textbf{RS} & \textsf{\footnotesize{}S}\textsf{\tiny{}inv} & \textsf{\footnotesize{}T}\textsf{\tiny{}inv} & \textbf{SAT} & \textsf{\footnotesize{}S}\textsf{\tiny{}inv} & \textsf{\footnotesize{}T}\textsf{\tiny{}inv} & \textbf{AR}\tabularnewline
\hline 
\hline 
Bakery \cite{ben2006principles,lynch1996distributed}  & 0.0s & 6 & 18 & 0.5s  & 2 & 5 & 0.0s \tabularnewline
\hline 
Burns \cite{abdulla2007regular}  & 0.2s & 8 & 96 & 1.1s  & 2 & 10 & 0.0s \tabularnewline
\hline 
Szymanski \cite{szymanski1988simple}  & 0.3s & 43 & 473 & 1.6s  & 2 & 21 & 0.1s \tabularnewline
\hline 
German \cite{german1992reasoning}  & 4.8s & 14 & 8134 & t.o. & \textendash{} & \textendash{} & 10s \tabularnewline
\hline 
Dijkstra \cite{abdulla2007regular}  & 0.1s & 9 & 378 & 1.7s  & 2 & 24 & 0.3s \tabularnewline
\hline 
Dijkstra ring \cite{dijkstra1984invariance,fribourg1997reachability}  & 1.4s & 22 & 264 & 0.9s  & 2 & 14 & 0.1s \tabularnewline
\hline 
Dining cryptographer \cite{chaum1988dining}  & 0.1s & 32 & 448 & t.o. & \textendash{} & \textendash{} & 7.2s \tabularnewline
\hline 
Gries's coffee can \cite{lin2016liveness}  & 0.0s & 3 & 18 & 0.2s  & 2 & 7 & 0.0s \tabularnewline
\hline 
Herman linear \cite{herman1990probabilistic}  & 0.0s & 2 & 4 & 0.2s  & 2 & 4 & 0.0s \tabularnewline
\hline 
Herman ring \cite{herman1990probabilistic}  & 0.0s & 2 & 4 & 0.4s  & 2 & 4 & 0.0s \tabularnewline
\hline 
Israeli-Jalfon \cite{israeli1990token}  & 0.0s & 4 & 8 & 0.1s  & 2 & 4 & 0.0s \tabularnewline
\hline 
Lehmann-Rabin \cite{lehmann1981advantages}  & 0.1s & 8 & 48 & 0.5s  & 2 & 11  & 0.0s \tabularnewline
\hline 
LR philosopher \cite{lin2016liveness}  & 0.0s & 4 & 16 & 0.2s  & 2 & 6 & 0.0s \tabularnewline
\hline 
mux array \cite{fribourg1997reachability}  & 0.0s & 5 & 30 & 0.4s  & 2 & 7 & 0.0s \tabularnewline
\hline 
Resource allocator \cite{donaldson2007automatic}  & 0.0s & 5 & 15 & 0.0s  & 1 & 3 & 0.0s \tabularnewline
\hline 
Kanban \cite{abdulla2013all,kaiser2010dynamic} & t.o. & \textendash{} & \textendash{} & t.o. & \textendash{} & \textendash{} & 3.5s\tabularnewline
\hline 
Water jugs & 0.1s & 24 & 264 & t.o. & \textendash{} & \textendash{} & 0.0s\tabularnewline
\hline 
\end{tabular}}
\end{center}
\vspace{-0.5cm}
\caption{\textbf{RS} is Rivest and Schapire's version of L{*},
\textbf{SAT} is the SAT-based enumeration, and 
\textbf{AR} is result of the ARTMC tool. 
Columns \textsf{\footnotesize{}S}\textsf{\tiny{}inv}
and\textsf{\footnotesize{} T}\textsf{\tiny{}inv} list the numbers
of states and transitions, respectively, in the obtained invariants.
Notations oom, t.o., and s.o. mean out-of-memory, time-out, and stack-overflow,
respectively.}
\vspace{-0.5cm}\label{tab:comp_tools}
\end{wraptable}
